YODA: Enabling computationally intensive contracts on blockchains with Byzantine and Selfish nodes

One major shortcoming of permissionless blockchains such as Bitcoin and Ethereum is that they are unsuitable for running Computationally Intensive smart Contracts (CICs). This prevents such blockchains from running Machine Learning algorithms, Zero-Knowledge proofs, etc. which may need non-trivial computation. In this paper, we present YODA, which is to the best of our knowledge the first solution for efficient computation of CICs in permissionless blockchains with guarantees for a threat model with both Byzantine and selfish nodes. YODA selects one or more execution sets (ES) via Sortition to execute a particular CIC off-chain. One key innovation is the MultI-Round Adaptive Consensus using Likelihood Estimation (MIRACLE) algorithm based on sequential hypothesis testing. M I RACLE allows the execution sets to be small thus making YODA efficient while ensuring correct CIC execution with high probability. It adapts the number of ES sets automatically depending on the concentration of Byzantine nodes in the system and is optimal in terms of the expected number of ES sets used in certain scenarios. Through a suite of economic incentives and technical mechanisms such as the novel Randomness Inserted Contract Execution (RICE) algorithm, we force selfish nodes to behave honestly. We also prove that the honest behavior of selfish nodes is an approximate Nash Equilibrium. We present the system design and details of YODA and prove the security properties of MIRACLE and RICE. Our prototype implementation built on top of Ethereum demonstrates the ability of YODA to run CICs with orders of magnitude higher gas per unit time as well as total gas requirements than Ethereum currently supports. It also demonstrates the low overheads of RICE.

==> sections/IntroTodo.tex <==
% !TEX root = ../main.tex
\section{New Introduction}

\sourav{The basic point of this part is to requirement of CICs}
\subsection{Part-I}
\begin{itemize}
	\item Brief introduction about blockchain(1-2 lines).
	\item Introduce the concept of smart-contract. Describe that smart contracts
	allows to have stateful executions in blockchains. (3-4 lines).
	\item Give an example of smart contract (2-party game).
	\item Motivating that smart contracts are useful entities to have, 
	its potential applications are huge.
	\item A large number of such smart contracts are potentially computationally
	heavy. 
	\item Mentioning that current blockchain systems are unsuitable 
	to execute such CICs. due to verifiers Dilemma. 
\end{itemize}

\subsection{Discussing the two naive extremes}

\sourav{First, the technique of dividing the program into multiple small programs}
As immediate mechanism to side-step the verifiers dilemma as mentioned in~\cite{luu2015demystifying} is too break the
computation into multiple blocks. Although Luu et al. considered a mechanism of breaking the program from end-user point
view, support from compilers can ease the process significantly from the point of view of user. One possible mechanism
would be build a compiler that allows to pause and store intermediate execution state of a program and resume it in
later blocks. Apart from the effort required to make this system secure by considering correct stop and pause semantics
there are quite a few problems that makes this approach un-suitable for the long run. First, the number of blocks that requires to compute a program grows linearly to the size of the computation. Additionally this is made worse by the
inter-arrival rate of blocks in the system. More fundamentally, even in this mechanism entire network executes the
contract leading drastically increasing the transaction making this design suitable for CIC.~\footnote{With current ethereum price and gas usage per insttuctions, a smart-contract consuming 1B gas will require a transaction fees of 0.5M USD.}

\sourav{Usage of zero knowledge techniques \miracle}

At the other extreme the most optimal way of solving the problem of CIC in blockchain is that a single node executes the CIC
and the remaining network has a mean of verifying whether the computation is correct. One immediate 
alternative that comes that comes to mind to achieve this to use techniques from cryptography that
allows a party to verify a computation without execution. Even though this seems promising, executing this
efficiently is an distant vision achieving which must fraught with several hurdles. All such schemes requires
pre-processing of computation that first requires an deep expertise of cryptography and there exist no 
general algorithm that can automate this for all kinds of programs written in high-level languages thus by hampering its 
usability. Second, often it is the case that solving this pre-processed system requires drastically more computation
raising an pragmatic concern to adoption of these scheme. Verification of the computation also becomes expensive. 
Additionally, this approach is vulnerable to single point of failure (both fail-stop and Byzantine) leading to significant
increase in time of computation in case of failures. 


After considering the issues at both the extremes one intuitive recourse is to use ideas from sharding.
\subsection{Part-II}

\sourav{Why sharding and why not?}

\begin{itemize}
	\item One might falsely assume that one can solve the problem of CICs using shards. There are quite a few problems with adopting sharding based systems. Few are of them are immediate and are fundamental to the design of sharding based system.
	\begin{enumerate}
		\item Sharding based systems generally consists a large number of nodes
		\item The traditional consensus approaches taken by this system requires the nodes
		in a shard to form an overlay network.
		\item Forming this overlay network could be an over-kill to the system and makes 
		these shards vulnerable to DoS attacks as their identities in the network are already known.
		\item Alternatively, creating shards on arrival of each CIC transactions will also be performance
		bottleneck ans the cost of forming a shard could be really expensive and will not scale for large number of
		CICs.
	\end{enumerate}

	There is a deeper class of problems that emphasizes that sharding based system are not suitable for CICs atleast with the
	current design. These includes
	\begin{enumerate}
		\item All these systems assume the non-Byzantines nodes to be honest i.e they strictly adhere to the protocol independent of immidiate incentives given to them. 
		\item The above assumptions might be hold true in situations where the cost of participating in consensus are very small and nodes earn block reward in sufficiently large interval. This can be justified since all block creations are expected to take equivalent amount of cost.
		\item However, this is not the case for CICs as the computation cost of each block may vary based on the running time of CICs embedded in it. As of current system, rewarding the leader will not be sufficient leader may engage into several spurious kinds of activities like creating large number of own CICs so as to include them in their block. This is a genuine attack as since the system is assumed to be incentive compatible, the net gain for executing each CICs needs to be positive. These hints us that arbitrary adoptions of existing rewarding scheme may not be suitable for CICs.
		\item The above discussion hints us that the gain in reward should not be in control of an individual in a single round. Additionally, for the system to be fair all nodes executing the CICs must earn equal reward at least with very high probability. 
	\end{enumerate}
\end{itemize}

\subsection{Choices of node behavior in the system}
\sourav{To highlight,  why considering both extremes of only rational and (honest+byzantine) is not appropriate}

\begin{itemize}
	\item At least, in case of CICs assuming all non-byzantine nodes are honest is not pragmatic.
	\item So does the idea of using all rational nodes.
	\item Introduce the concept of BAR Byzantine, Altruistic and Rational nodes in a system.
	\item Why this is difficult to study. 
	\item We dont claim to solve the problem of BAR completely due to various reasons.
		\begin{enumerate}
			\item First, it is difficult to design the notion of utility in general setting. 
			\item This notion of utility becomes much more challenging if one decides to that are beyond the control
			of the protocol designer. This includes \em{Gold Finger attack}, \em{Feather-forking attack} etc.
		\end{enumerate}
	\item We take a step closer to design a system comprising of byzantine and rational nodes by first, defining a utility
	model that may not accurate, designing the protocol in the manner that only allows honest nodes to make limited 
	deviations from the honest behavior. Defining a reward scheme that ensures honest-behavior of rational
	node is an approximate-Nash equilibrium. 
\end{itemize}


\subsection{Performance of the system}
\sourav{Motivation why performance is a point one must consider while design.}
As executing each CICs are expensive, lower the repetition of CICs better is the performance of the system. 
Various mechanisms enabling CICs in a permissionless blockchain in a BAR threat model can be intuitively compared. 
Mechanism that can provide security with lower repetition of execution can be deemed better. 
It was not clear on how to reduce the size of the set repeating the execution until we hit upon a very crucial
point on adversarial fraction of nodes present in the system that is often missed by other design. 
All existing protocols in this blockchain start with a threat model considering some $f_{max}$ fraction of adversarial
control in the system and their protocols are designed tolerate up to $f_{max}$ fraction of the nodes. 
However, it is $f_{max}$ is a worst case scenario and pragmatic experience hints that often actual adversarial
fraction could be possibly low. There lies a implicit trade-off between security and performance of these
protocol and all protocols compromise performance to guarantee against worst case security. 

The insight is good, but however at the earliest stage of our design it was not clear how to take advantage
of the fact that adversarial fraction of nodes may be lower than $f_{max}$. The major bottleneck was to 
identify the actual fraction of adversarial control. Reputation systems seems plausible direction but note
that an intelligent adversary can easily defeat it by simply following the protocol prior to an attack.
Alternatively since blockchains often embedded economic values in it any such protocols needs to be 
proactive i.e must identify attack on it and adapt appropriately. 

A consistent quest for such protocol led us to design of our novel Multi-round Adaptive Consensus Using 
Likelihood estimations~(MiRACLE) that we describe in detail in~\textsection{sec:miralce}.

\subsection{Overview of YODA and Contributions} 
In this paper we present YODA, which is to the best of our knowledge
the first solution for efficient computation of CICs in permissionless
blockchains which gives security guarantees in a BAR threat model. The
threat model allows a fraction of Byzantine nodes $f\le f_{max}<0.5$
in the overall system and the remaining can be {\em quasi-honest}. Quasi-honest nodes are
selfish nodes which seek to maximize their utility by skipping CIC
computation using information about its solutions which may already be
published on the blockchain by other nodes, an attack termed a {\em free-loading attack}. 
% {\bf VINAY: WE NEED TO BE CONSISTENT IN DEFINTION. ARE QUASI-HONEST NODES ALLOWED TO COLLUDE OR NOT?} 
They may also try to collude with each other to reduce their computation. The assumptions on quasi-honest nodes are given in detail in \textsection \ref{sub:threat assumption}.
%  YODA has a working prototype implementation
%based on Ethereum.  
It is robust to DoS attacks, Sybil attacks, and
ensures timely payouts to all who execute a CIC.

YODA's modus operandi is to make only small sets of randomly selected
nodes called Execution Sets (ES) execute the CICs. ES nodes submit
their solutions on the blockchain as a transaction and YODA must thus identify the
correct solution from among them. Note that this problem is not the
same problem of  achieving consensus about blocks in the blockchain using
shards \cite{luu2016secure, kokoris2017omniledger,
  al2017chainspace,gilad2017algorand}.  Blocks can in general take
many valid values and are computationally easy to verify unlike CIC solutions
which have only one correct value and are computationally expensive to verify.


Because CICs are
not executed by all nodes, we say they are always computed {\em
  off-chain}, as opposed to other smart contracts which are said to be
executed {\em on-chain} by all miners. While a small ES improves
system efficiency, it can occasionally be dominated by Byzantine nodes
which may form a majority and submit incorrect solutions. Hence a simple majority decision
does not work even in a setting with only honest and Byzantine nodes.

Our first major contribution is the {\em MultI-Round Adaptive
  Consensus using Likelihood Estimation} (MiRACLE) which addresses
this problem. It is adaptive to the fraction $f$ of Byzantine nodes in the system in the following fashion.
MiRACLE is designed so that in case most of the ES nodes
submit the same solution (which happens when the fraction of Byzantine nodes is small, i.e. $f\ll f_{max}$), it is correct with high probability and the
submitted solution is immediately accepted by miners. However, in case no single
solution is the clear winner, a second random ES is chosen to start a
new 
{\em round},\footnote{rounds are different from block-generation epoch and are specific to CICs. A round may span multiple blocks} and so on. This latter case happens more often when $f$ is close to $f_{max}$, that is the fraction of Byzantine nodes is large.
Hence data comes in sequentially from one
ES after the other. 

We present a novel formulation of this problem as a multiple hypothesis testing problem where we have one hypothesis for each
solution submitted and the test must decide which hypothesis is true. The winning hypothesis decides the solution. 
This model is not obvious because traditional hypothesis testing, for example for signals in noise, deal with real world
artifacts with known probability distributions, and not intelligent adversaries who can behave arbitrarily. 


MiRACLE  uses multiple parallel
 Sequential Probability Ratio
Tests (SPRT) to choose the correct solution \cite{wald1973sequential}.

MiRACLE guarantees that the correct solution is chosen with
probability set by a design parameter in the worst case of
$f=f_{max}$.  Moreover, MiRACLE is optimal in that it minimizes the
expected number of rounds in the special case that all Byzantine nodes
submit the same incorrect solution and $f=f_{max}$. Interestingly, the
optimal strategy for Byzantine nodes to make MiRACLE accept an
incorrect solution is to submit the same incorrect solution. Our
analysis for MiRACLE, however, assumes quasi-honest nodes submit
correct solutions. Since MiRACLE itself does not enforce honest behavior
other mechanisms are necessary to make quasi-honest nodes submit correct solutions.
Without additional mechanisms,
a quasi-honest node may be tempted to free-load on solutions of earlier rounds, thus
rendering our analysis for MiRACLE invalid. 
Although we present MiRACLE in the context of CIC execution, it can be used in a broader suite of security problems,
some of which we describe in \textsection \ref{sub:miracle applications}.

Our second contribution is the {\em Randomness Inserted Contract
  Execution} (RICE) algorithm which deliberately adds randomness to
the solution of each round so that the CIC solution changes from one
round to the next thereby mitigating the free-loading attack.  We
prove that no matter the size of the CIC computation, RICE adds little
computational overhead. To be precise, if $T$ denotes the
total computation for a transaction execution without RICE, then RICE
adds computation overhead of the $O((log_2 T)^2)$. In the
presence of free-loading attacks, we show via a game theoretic
analysis that honest behavior from all quasi-honest nodes is an $\epsilon-$Nash
equilibrium with $\epsilon\ge 0$.

The third contribution is an implementation of YODA in
Ethereum using the geth Client interface version \texttt{1.8.7}.
The implementation includes MiRACLE, RICE, and most other features of YODA. 
% All CICs are implemented on the blockchain
% as part of a {\em Master Contract} (MC).
% The MC contains one queue for each smart contract to order transactions of a CIC.
Using a testbed consisting of 8 physical machines emulating 1600
nodes, we compare the performance of YODA with that of Ethereum in
terms of the gas usage possible per unit time as well as the total gas
usage of contracts.  We also study the number of rounds for MiRACLE to
converge for different design parameters. We show how MiRACLE
automatically reduces the number of rounds if the fraction of
Byzantine nodes is less than the worst case design scenario. We also
show that RICE hardly adds any overhead to the CIC computation.

Other contributions are several mechanisms in YODA to make it robust to attacks
such as chain forking attacks (CFA), DoS attacks, and Sybil attacks,
and collusion attacks. These mechanisms include
using Sortition along with
commitments and incentives. We provide a game theoretic analysis
for a collusion attack by quasi-honest nodes which 
increase their utility by sharing information using recent
advancements in zk-Techniques \cite{ben2014succinct}. We show that
the game has a $\delta-$ Nash Equilibrium.

These are added
contributions which may be of interest to the reader.

{\bf Paper Organization:} In Section \ref{sec:system design} we present a
system overview of YODA and mention requirements for off-chain execution. This is followed by the Threat Model
and an overview of Challenges in Section \ref{sec:threat}.
In Section \ref{sec:miracle} we present
the MiRACLE algorithm followed by a detailed description of RICE
in Section \ref{sec:rice}.
We then put all ingredients together to describe the YODA protocol
in Section \ref{sec:enabling cic}
followed by a Security
Analysis in Section \ref{sec:analysis}. We then present details of
our Ethereum-based implementation along with experimental results in
Section \ref{sec:eval}. Section \ref{sec:related} describes related
work. We conclude with a discussion in Section \ref{conclusion}.


\subsection{Challenges}
\label{sub:challenges}
%Enabling off-chain execution of CICs in the presence of a  Byzantine adversary is fraught with many challenges. Allowing non-Byzantine nodes to deviate from protocol makes the problem more interesting and even more challenging. 
Apart from recently studied challenges like preventing {\it Sybils} in SP \cite{nakamoto2008bitcoin,pob} and generating an unbiased source of randomness in the distributed setting to select ES randomly \cite{gilad2017algorand,luu2016secure,syta2017scalable}, our system must tackle the following. The first challenge is to prevent quasi-honest nodes from {\em Free-loading and collusion}. 
%Because in MiRACLE, solutions of the CIC have already been published by ES sets of earlier rounds, an ES node of the current rounds may be tempted
%to replay the highest occurring solution\footnote{In certain cases the highest occurring solution is not most likely to be correct. Details are given in Section \ref{sec:miracle}} among these, as this is likely to be the correct solution with highest probability among solutions submitted. This is called the free-loading attack. A collusion attack is one in which quasi-honest nodes group together
%to submit a solution which maximizes their rewards while reducing individual computation.
The second challenge is that since ES size is small, they become vulnerable to {\it Lower cost DoS Attacks} than a DoS attack on the entire blockchain network. 

Further, existing on-chain verification of off-chain computation methods fall into two
categories: Symmetric and Asymmetric. In symmetric methods, a  contract is re-executed on-chain by miners and is hence its computation is limited due to the Verifiers Dilemma. 
In the asymmetric model, the on-chain verification  uses a method other than recomputation, either by generating a proof-of-execution, possibly interactive \cite{teutsch2017scalable}, or via non-interactive methods using zk-SNARK \cite{ben2014succinct}. These techniques are associated with non-deterministic overheads (depending upon the CIC) (eg. Truebit) or are too computationally expensive for general purpose hardware. Designing a verification scheme that adds a small constant computational overhead of on-chain verification, independent of the CIC is new. We are the first to take this approach. Also, since CICs are never executed on-chain, producing both efficient off-chain  execution and providing guarantees of correctness is challenging.


